Generalized Group Data Attribution

Data Attribution (DA) methods quantify the influence of individual training data points on model outputs and have broad applications such as explainability, data selection, and noisy label identification. However, existing DA methods are often computationally intensive, limiting their applicability to large-scale machine learning models. To address this challenge, we introduce the Generalized Group Data Attribution (GGDA) framework, which computationally simplifies DA by attributing to groups of training points instead of individual ones. GGDA is a general framework that subsumes existing attribution methods and can be applied to new DA techniques as they emerge. It allows users to optimize the trade-off between efficiency and fidelity based on their needs. Our empirical results demonstrate that GGDA applied to popular DA methods such as Influence Functions, TracIn, and TRAK results in upto 10x-50x speedups over standard DA methods while gracefully trading off attribution fidelity. For downstream applications such as dataset pruning and noisy label identification, we demonstrate that GGDA significantly improves computational efficiency and maintains effectiveness, enabling practical applications in large-scale machine learning scenarios that were previously infeasible.

==> neurips_format/abstract.tex <==
Data Attribution (DA) methods quantify the influence of individual training data points on model outputs and have broad applications such as explainability, data selection, and noisy label identification. However, existing DA methods are often computationally intensive, limiting their applicability to large-scale machine learning (ML) models. 
To address this challenge, we introduce the Generalized Group Data Attribution (GGDA) framework, which computationally simplifies DA by attributing to groups of training points instead of individual ones. GGDA is a general framework that subsumes existing attribution methods and can be applied to new DA techniques as they emerge. It allows users to optimize the trade-off between efficiency and fidelity based on their needs. Our empirical results demonstrate that GGDA applied to popular DA methods such as Influence Functions, TracIn, and TRAK results in up to \textbf{10x-50x} speedups over standard DA methods while gracefully trading off attribution fidelity. For downstream applications such as dataset pruning and noisy label identification, 
we demonstrate that GGDA significantly improves computational efficiency and maintains effectiveness, enabling practical applications in large-scale ML scenarios that were previously infeasible.%\footnote{Code is available at \textit{<anonymized>}}


% \textcolor{red}{Hima to work on abstract}
% Data attribution (DA) measures the influence of training data to model outputs, which has broad applications in data selection, mislabel detection, copyright compensation, and many more. However, these methods are often computationally intensive, limiting their applicability to large-scale machine learning models. In this paper, we introduce the Generalized Group Data Attribution (GGDA) framework, a generalization that computationally simplifies DA by attributing to groups of training points instead of individual ones. GGDA subsumes the existing attribution methods into a general framework. Our empirical results of GGDA applied to popular DA methods such as influence functions, TracIn, and TRAK demonstrate result in orders-of-magnitude speedups over standard DA methods while gracefully trading off attribution fidelity. For downstream applications such as dataset pruning and noisy label identification, we find that the GGDA outperforms and matches standard DA methods while providing significant speedups.\footnote{Code is available at $<$anonymous link$>$.}    

% \sz{Suggestions from the group meeting

% - Clarify that DA produces scores, these scores can be used for different applications, add concrete and well-known data attr methods (in the first 2 sentences)

% -  Emphasize that GGDA subsumes other DA methods as a general framework

% - GGDA is general. For new methods, we can also apply GGDA on them.

% - What we propose (can work in more general cases, including Shapley-based methods) vs. what we experiment on (More specific methods, IF-based, talk about them when we mention empirical results)
% }

% Data attribution (DA) analyzes machine learning models in terms of their training data by identifying important training points that impact individual model outputs. However, these methods are computationally intensive, limiting their applicability to large-scale machine learning models. To address this, we introduce the Generalized Group Data Attribution (GGDA) framework, a generalization that computationally simplifies DA by attributing to groups of training points, subsuming the DA framework of attributing to individual points. We then propose GGDA generalizations of three Influence function-based methods (LiSSA, Fisher, and TracIn) with runtime benefits over their DA variants due to grouping. Our empirical results demonstrate that GGDA-based influence methods result in orders-of-magnitude speedups over standard DA methods while gracefully trading off attribution fidelity. For downstream applications such as dataset pruning and noisy label identification, we find that the GGDA generalizations significantly outperform standard DA methods while providing significant speedups.  




%Data attribution methods are increasingly being considered for identifying instances that impact aggregate behaviors of models (e.g., accuracy, fairness etc)
% However, one of the key drawbacks of these methods is that they are computationally intensive and are not practical
%To address these challenges, we introduce the Generalized Data Attribution framework which takes a new perspective of group-level data attributions instead of instance-level data attributions. 
%To this end, we first unify three popular data attribution methods and establish the connections between them via different Hessian approximations. We then extend this to generate group-level data attributions. We further leverage the closed-form solutions proposed in data-inf paper to improve the efficiency of our method and outline strategies for choosing groups that can effectively capture attribution pertaining to specific aggregate behaviors (e.g., accuracy, fairness). 
%empirical results demonstrate that the estimate's accuracy vs. efficiency frontier is much better with our method. 
  

==> neurips_format/experiment.tex <==
This section presents highlights from a comprehensive evaluation of our proposed GGDA framework.
We conduct experiments on multiple datasets using various models to demonstrate the effectiveness and efficiency of our approach compared to existing data attribution methods.
We evaluate across four diverse datasets encompassing tabular (HELOC), image (MNIST and CIFAR-10), and text data (QNLI).
These datasets represent a range of task complexities, data types, and domains, allowing us to assess the generalizability of our approach across different scenarios.
The models we fit on these datasets range from simple logistic regression (LR) to medium-sized artificial neural networks (ANNs, e.g., MLPs and ResNet) and pre-trained language models (BERT). %See Appendix~\ref{subapp:datasetsmodels} for detailed dataset descriptions and model hyperparameters.% Further details can be found in Appendix~\ref{subapp:datasetsmodels}.
Full configuration details for datasets, models, attribution methods, grouping methods, and evaluations are listed in Appendix~\ref{app:setup}, while the remainder of results across our grid of experiments is in Appendix~\ref{app:results}.

\subsection{Grouping Methods}
\label{subsec:grouping}

We employ several grouping methods to evaluate the effectiveness of our GGDA framework. For each grouping method, we also experiment with various group sizes to analyze the trade-off between computational efficiency and attribution effectiveness.
The choice of grouping method and group size can significantly impact the performance of GGDA, as we subsequently demonstrate.% in our subsequent experiments (Section~\ref{subsec:results}). %We refer full clustering setup and hyperparameters to Appendix~\ref{subapp:grouping}

% \begin{compactitem}[\textbullet] 
Groupings comprise of: \textbf{Random}, assigning data points to groups of a specified size uniformally randomly (serving as a baseline); \textbf{K-Means}, grouping data points based on raw features; \textbf{Representation K-Means (Repr-K-Means)}, grouping data points on hidden representations from the model we attribute on, capturing higher-level semantic similarities; and \textbf{Gradient K-Means (Grad-K-Means)}, grouping on the gradient of the loss wrt activations (NOT parameters) of the pre-classification layer of the model, grouping instances with similar effects on the model's learning process.

\subsection{Evaluation Metrics}

To illustrate the effectiveness of GGDA at identifying important datapoints, in comparison to DA, it is critical to have metrics that allow us to compare both on equal terms. To this end, we utilize:

\textbf{Retraining Score (RS)}\hspace{5pt} This metric quantifies the impact of removing a proportion of training data points on model performance.
The process involves (1) identifying the most influential groups using GGDA, (2) removing a given percentile of high-importance points, (3) retraining the model, and (4) comparing the performance of this model to the original model's performance on the test set.
A significant decrease in performance (i.e., an increase in loss or decrease in accuracy) indicates that the removed points were indeed important for the model's learning process.
This metric provides a tangible measure of the effectiveness of GGDA in identifying highly useful training instances.

% \textbf{Dataset Pruning}\hspace{5pt} \dan{uses retrain score on least important points: 25\%, 50\%, 75\%}

\textbf{Noisy Label Detection (AUC)}\hspace{5pt} This metric quantifies the effectiveness with which GGDA methods can identify mislabelled training data points. This involves randomly flipping a proportion of the training set labels, and training a model on the corrupted dataset.
We then examine the labels of the training data points that belong to groups with the lowest scores, and plot the change of the fraction of detected mislabeled data with the fraction of the checked training data, following \cite{ghorbani2019data, jia2021scalability}. The final metric is computed as the area under the curve (AUC). %Exact implementation details and example curves are displayed in Appendix~\ref{subapp:noisy}.



% \subsection{Experimental Setup}

% For each dataset and model combination, we use grid search to optimize key parameters such as learning rates (ranging from 1e-5 to 1e-2), batch sizes (32 to 256), and model-specific hyperparameters.
% For our GGDA method, we explore various group sizes (1, 4, 16, 64, 256, 1024) and grouping strategies (Random, K-Means, Repr-K-Means, Grad-K-Kmeans) to analyze their impact on attribution quality and computational efficiency. 

\subsection{Results}
\label{subsec:results}

In the following subsections, we present results from across our range of datasets and models, discussing GGDA performance in terms of retraining score, computational efficiency, and effectiveness in downstream tasks such as dataset pruning and noisy label detection.
Our pipeline trains a model on the full training set and determines groups as described in Section~\ref{subsec:grouping}. We ablate extensively over a range of group sizes, beginning at 1 (standard DA) and increasing to 1024, in ascending powers of 2.

% We pay particular attention to how our method scales across different data modalities and model complexities, from simple logistic regression on tabular data to large language models on text data.

\subsubsection{Retraining Score}

To evaluate the retraining score metric, we compute \textit{Test Accuracy} upon removal of 1\%, 5\%, 10\%, and 20\% of the most important points in the train set. For groups, this translates to sequentially removing the most important groups up until the desired number of data points (points are randomly selected from the final group in the case of overlap). Lower test accuracies are thus more favorable.

\begin{figure}[t]
    \centering
    \includegraphics[width=0.95\linewidth]{figures/retrain_grouping2/mnist_ann_l_20_accuracy_performance_vs_runtime.pdf}
    \caption{\small \textbf{Ablation over grouping methods.} Test accuracy (\%) retraining score on MNIST after removing the top 20\% most important training points (lower is better). Grad-K-Means grouping is superior, achieving comparable performance to individual attributions at orders of magnitudes faster runtime. Error bars represent standard error computed on 10 differently seeded model retrainings.}
    \label{fig:retrain_grouping_mnist}
\end{figure}
\begin{figure}[b]
    \centering
    \includegraphics[width=0.95\linewidth]{figures/retrain/cifar10_resnet18_grad_kmeans_accuracy_performance_vs_runtime.pdf}
    \caption{\small \textbf{GGDA attribution fidelity across removal percentages}. Test accuracy (\%) retraining score using Grad-K-Means grouping on CIFAR-10 after removing 1\%, 5\%, 10\%, and 20\% of the most important points (lower is better). GGDA methods save orders of magnitude of runtime while gracefully trading off attribution fidelity. See Appendix~\ref{subapp:retrain} for similar findings across all datasets and models.}
    \label{fig:retrain_cifar10}
\end{figure}

\textbf{Which Grouping Method to Use?}\hspace{5pt} We plot a subset of group sizes that decreases from left to right as runtimes simultaneously increase, until GGDA subsumes DA at size 1. We find that across the board, Grad-K-Means most consistently demonstrates superior performance. Figure~\ref{fig:retrain_grouping_mnist} illustrates this for MNIST (similarly conclusive plots for remaining datasets and models are in Appendix~\ref{subapp:retrain}).

\textbf{Results across Removal Percentages.}\hspace{5pt} Based on our results above, we employ Grad-K-Means as the primary grouping method, and trial incremental increases on the removal percentage for the retraining metric (using values of 1\%, 5\%, 10\%, 20\%). Our results in Figure~\ref{fig:retrain_cifar10} show that GGDA, in general, has a favorable accuracy efficiency tradeoff. In particular, we find that the performance levels are roughly equivalent across group sizes $\{1,4,16,64\}$, but with orders-of-magnitude speedup.

%\dan{Last remaining todo:} Figure~\ref{fig:retrain_cifar10} demonstrates representative results. Approximate equivalency to individual DA methods but with orders of magnitude runtime when considering group sizes 1, 4, 16, 64.

% Group attributions in general have favorable accuracy efficiency tradeoff.

% Figure~\ref{fig:retrain_cifar10}

% \subsection{Downstream Applications}

\subsubsection{Dataset Pruning}

To evaluate the effectiveness of GGDA in dataset pruning, we compute \emph{test accuracy} after removing varying percentages (25\%, 50\%, 75\%) of the least important points from the training set (retraining score). Higher test accuracies after pruning are more favorable.
Our results demonstrate that GGDA significantly outperforms individual DA methods in this task, achieving higher test accuracies while requiring substantially less compute. Table~\ref{tab:pruning_tracin} presents example results for a range of datasets using TracIn, illustrating the superior performance and efficiency of GGDA compared to individual DA.%~\ref{tab:pruning_heloc_lr} and

% \textbf{Takeaway:} GGDA significantly outperforms individual DA. Example results are shown in Table~\ref{tab:pruning_mnist}.

% We show TracIn, which performed best, for MNIST / CIFAR-10 / QNLI in Table~\ref{tab:pruning_tracin}.
% Alternatively, display in tables, select from the following, move rest to Appendix:


% \input{tables/pruning/heloc_lr_random_1024}
\input{tables/pruning/tracin_random_1024}

% \begin{table}[h]
% \caption{Test accuracies (\%) after pruning the MNIST dataset with varying removal percentages and for various DA/GGDA methods. }
% \label{sample-table}
% \begin{center}
% \begin{tabular}{ccccccc}
% &\multicolumn{2}{c}{\bf TracIn}  &\multicolumn{2}{c}{\bf Influence (Fisher)} &\multicolumn{2}{c}{\bf Influence (LiSSA)} \\
% Removal \% & DA & GGDA & DA & GGDA & DA & GGDA \\
% \midrule
% 25\% & 95.8 ± 0.1 & 97.5 ± 0.0 & 96.7 ± 0.1 & 97.4 ± 0.0 & 96.0 ± 0.1 & 97.4 ± 0.1 \\
% 50\% & 93.6 ± 0.2 & 97.1 ± 0.1 & 96.3 ± 0.1 & 97.1 ± 0.1 & 94.0 ± 0.3 & 97.0 ± 0.1 \\
% 75\% & 85.8 ± 3.3 & 96.1 ± 0.1 & 95.6 ± 0.1 & 95.9 ± 0.1 & 92.6 ± 0.6 & 95.9 ± 0.1 \\
% \midrule
% Runtime (s) & 311.0 & 6.6 & 227.3 & 5.1 & 306.9 & 25.9 \\ \bottomrule
% \end{tabular}
% \end{center}
% \end{table}

% \begin{figure}
%     \centering
%     \includegraphics[width=0.95\linewidth]{figures/pruning/heloc_ann_m_equal_accuracy_performance_vs_runtime.png}
%     \includegraphics[width=0.95\linewidth]{figures/pruning/mnist_ann_l_equal_accuracy_performance_vs_runtime.png}
%     \includegraphics[width=0.95\linewidth]{figures/pruning/cifar10_resnet18_old_equal_accuracy_performance_vs_runtime.png}
%     \includegraphics[width=0.95\linewidth]{figures/pruning/qnli_bert_equal_accuracy_performance_vs_runtime.png}
%     \caption{\dan{NOTES: Pick graphs we want. Put dataset names sideways on LHS. HELOC LR/ANN\_S look similar to ANN\_M. Should make a plot showing where GGDA methods outperform- a bar plot perhaps.}}
%     \label{fig:pruning_main}
% \end{figure}

\subsubsection{Noisy Label Identification}

Noisy label detection is a critical task in ML, addressing inaccurate labelling in real-world datasets.
We analyze the trade-off between detection accuracy (AUC) and computational efficiency (runtime).
We present our findings for CIFAR-10 and QNLI in Table~\ref{tab:noisy}, demonstrating superior performance for GGDA, with the remainder in Appendix~\ref{subapp:noisy}. %Our analysis reveals several key findings regarding the performance of different DA methods in noisy label detection.
For BERT models, the Fisher approximation variant of influence functions shows improved performance when combined with grouping, while also reducing runtime by an order of magnitude.
TracIn demonstrates superior performance on the CIFAR-10 dataset, particularly when grouping datapoints with similar penultimate-layer gradients.
%However, we observe that TRAK performs poorly within the given computational budget, and methods like LiSSA show less pronounced group-wise speedups due to other computational bottlenecks. Nevertheless, applying GGDA to all of these DA methods improves their efficiency.%, which can potentially be due to the number of ensembles being small (10 ensembles in our case). We choose not to further increase the ensemble as retraining make TRAK much slower compared to ours and all the baselines. Increasing it makes these DA methods not really comparable in terms of run time. Also, 
% These results highlight the effectiveness of GGDA in enhancing both performance and efficiency across various datasets and model architectures.

\input{tables/noisy}

% \begin{figure}
%     \centering
%     \includegraphics[width=0.32\linewidth]{figures/noisy/heloc_noisy_ann_m_group_auc_vs_runtime.pdf}
%     \includegraphics[width=0.32\linewidth]{figures/noisy/mnist_noisy_ann_l_group_auc_vs_runtime.pdf}
%     \includegraphics[width=0.32\linewidth]{figures/noisy/cifar10_noisy_resnet18_group_auc_vs_runtime.pdf}
%     \caption{Main results for noisy label detection \dan{add caption, fix xticks and legend}. Notes: uses grad\_kmeans, group sizes 1, 4, 16, 64 plotted for clarity.}
%     \label{fig:noisy_main}
% \end{figure}

% Labels in the real world are often noisy due to automatic labeling, non-expert labeling, or label corruption by data poisoning adversaries.




==> neurips_format/future.tex <==
In this work, we have proposed a new framework, Generalized Group Data Attribution (GGDA), that offers computational advantages over data attribution while maintaining similar fidelity. While our work focuses on influence-based approaches, any data attribution approach can, in principle, be extended to the group setting to obtain these computational benefits. The key insight here is that many downstream applications of attribution involve manipulating training datasets at scale, and a fine-grained approach of individual point influence may be unnecessary in such cases.

There are several exciting avenues for future work. First, it is desirable to conduct a formal analysis of the fidelity tradeoffs in the group setting for various methods of interest. Second, while our experiments focus on small-to-medium-scale settings to systematically demonstrate the advantages of group attribution, evaluation on a genuinely large-scale, billion-data-point learning setting can help uncover any remaining computational bottlenecks limiting the practical adoption of data attribution.

==> neurips_format/introduction.tex <==
In the era of data-driven ML, the impact of training data on model performance has become increasingly evident.
% As such, the ability to discern and quantify the influence of individual training examples on model behavior has emerged as a critical area of research.
Data Attribution (DA) methods have risen as powerful tools designed to address this, identifying the influence of each training data point for specific predictions, offering insights into the relationships between training data and model behavior~\citep{koh2017understanding,ghorbani2019data, pruthi2020estimating, schioppa2022scaling, jia2021scalability, kwon2022beta, ilyas2022datamodels, park2023trak, wang2023data}.
DA applications are far-reaching, encompassing model debugging, strategic data selection, and mislabelled data detection. Existing techniques, however, incur prohibitive computational costs, e.g., by requiring retrainings in the order of the training data size (intractable for large-scale models~\citep{ghorbani2019data, ilyas2022datamodels}), and often struggle to faithfully represent the true impact of training data on model outcomes~\citep{basu2020influence}. %, which can lead to misinterpretations and potentially misguided model development and deployment decisions.
Efficiency and fidelity issues combined have severely restricted widespread adoption in large-scale applications.

To address these, we propose Generalized Group Data Attribution (GGDA), a framework that shifts the paradigm from attributing influence to individual data points to considering meaningful groups of data points collectively, enabling GGDA to substantially reduce computational overhead and making it particularly well-suited for large-scale applications where traditional DA methods falter. 
% Importantly, this improvement in efficiency comes at little cost to attribution fidelity.
% Overall, this framework improves the scalability of individual-point attribution techniques while maintaining and, in some cases, improving attribution fidelity. 
%GGDA is a flexible and general framework that extends any DA algorithm to the group setting, including Influence Functions~\citep{koh2017understanding}, TracIn~\citep{pruthi2020estimating}, and TRAK~\citep{park2023trak}.
%By adapting these methods to operate on groups of data points, GGDA significantly enhances computational efficiency.
% GGDA also offers a unique advantage in allowing users to fine-tune the trade-off between efficiency and fidelity through adjustable group sizes.
% This adaptability empowers practitioners to optimize the balance between computational efficiency and attribution fidelity based on their specific requirements.
%When the group size is set to one, GGDA reduces to the original DA method, thus it naturally subsumes a broader range of DA techniques as a general framework.
%sents a general solution that can work with existing methods, offering a comprehensive approach to improving both the efficiency and applicability of DA techniques. \suraj{Lots of content overlap with previous paragraph, potentially merge both and shorten?}
To validate the effectiveness of GGDA, we conduct extensive experimental evaluations across various datasets, model architectures, and DA methods.
Our results show that: (1) GGDA significantly improves the computational efficiency of DA methods, resulting in upto \textbf{10x-50x} speedups depending on the setting, (2) GGDA favourably trades off fidelity with efficiency compared to standard DA approaches, and (3) For downstream applications such as dataset pruning and noisy label identification, GGDA outperforms standard DA methods, while maintaining significant speedups.
%This advantageous balance enables the practical application of DA techniques in large-scale machine learning scenarios that were previously computationally prohibitive.


==> neurips_format/method.tex <==
We first show how to generalize Influence Functions to the GGDA setting, following two principles:
%In particular, we derive GGDA variants of gradient-based influence methods, given their inherent computational superiority over re-training-based methods.
% There are two principles we follow: 
\begin{compactitem}[\textbullet]
    \item the GGDA variants must scale with $k$, the number of groups, and not $n$, the number of datapoints;
    \item the GGDA variants must subsume the ordinary DA variants when groups are defined as singleton datapoints, and the property function as the loss on a single test point.
\end{compactitem}

\paragraph{Generalized Group Influence Functions.} Given a loss function $\ell \in \R^+$, Influence GGDA is:%the Influence Function data attribution method~\citep{koh2017understanding} is given by:

\begin{align*}
    \tau_\text{inf}(\mathcal{A}, \mathcal{D}, \X_\text{test}) = \underbrace{\nabla_{\theta} \ell(\X_\text{test}; \theta)^\top}_{\R^{1 \times p}}~ \underbrace{H_{\theta}^{-1}}_{\R^{p \times p}} ~ \underbrace{\big[ \nabla_{\theta} \ell(\X_0; \theta); \nabla_{\theta} \ell(\X_1; \theta); ... \nabla_{\theta} \ell(\X_n; \theta) \big]}_{\R^{p \times n}} ~~~~\theta \sim \mathcal{A}(\mathcal{D})
    %\label{eqn:inf}
\end{align*}

The primary computational bottlenecks for computing influence functions involve (1) computing the Hessian inverse, and (2) computing the $n$ gradients terms, which involve independent $n$ forward and backward passes.
%While several influence approximations \citep{guo-etal-2021-fastif, schioppa2022scaling} focus on alleviating the bottleneck due to computing the Hessian inverse, here we focus on the latter bottleneck of requiring order $n$ compute.
% While efficient computation of per-sample gradients has received attention from the machine learning community~\cite{jax2018github} via tools such as \texttt{vmap}, the fundamental dependence on $n$ remains, leading to large runtimes.
In Appendix \ref{app:gg-inf}, we show that due to linearity of influence functions, group influence is given by the sum of individual influences. %, which is consistent with the analysis in \cite{koh2019accuracy}.
The corresponding GGDA generalization is:
\begin{align}
    \tau_\text{inf}(\mathcal{A}, \mathcal{D}, \mathcal{Z}, g) &= \underbrace{\nabla_{\theta} g(\theta)^\top}_{\R^{1 \times p}}~ \underbrace{H_{\theta}^{-1}}_{\R^{p \times p}} ~ \underbrace{\big[ \nabla_{\theta} \ell(\Z_0; \theta); \nabla_{\theta} \ell(\Z_1; \theta); ... \nabla_{\theta} \ell(\Z_k; \theta) \big]}_{\R^{p \times k}} ~~~~~~\theta \sim \mathcal{A}(\mathcal{D}) \label{eqn:group_inf}
\end{align}

where $\ell(\Z_i) := \sum_{\X \in \Z_i} \ell(\X)$. From equation \ref{eqn:group_inf}, we observe that the corresponding group influence terms involve \ul{$k$ batched gradient computations} instead of \ul{$n$ per-sample gradient computations}, where all $\sim n/k$ points belonging to each group are part of the same batch. Typically, $k<<n$, leading to considerable overall runtime benefits for GGDA influence functions. We use this key insight for two more methods: TracIn and TRAK (presented in Appendix~\ref{app:derivations}).%, by viewing them as special cases of influence methods, even though this differs with the original motivation presented in these papers.

==> neurips_format/motivation.tex <==
\newtheorem{defn}{Definition}
This section introduces formal DA definitions. We examine limitations of conventional methods which attribute to individual points, showing that they often result in prohibitive computation. We then present the rationale behind Generalized Group Data Attribution (GGDA) as a solution.

\textbf{Notation.} Given a dataset of $n$ training data points $\mathcal{D} = \{ (\X_0, \Y_0), (\X_1, \Y_1), ... (\X_n \Y_n)\}$ in the supervised learning setting,\footnote{This can be easily extended to unsupervised learning.} and a learning algorithm $\mathcal{A}(\mathcal{D}): 2^{\mathcal{D}} \rightarrow \R^p$ that outputs weights $\theta \in \R^p$, where $f(\X_\text{test}; \theta) \in \R$ is the model prediction function for a given test input $\X_\text{test}$, we define a counterfactual dataset $\mathcal{D}_S = \mathcal{D} \setminus \{(\X_i, \Y_i; i \in S)\}$ as the training dataset with points in $S$ removed. We use $\theta_S \sim \mathcal{A}(\mathcal{D}_S)$ to denote the model weights trained on $\mathcal{D}_S$. 

\begin{defn}
    (Data Attribution) 
    Given a learning algorithm $\mathcal{A}$, dataset $\mathcal{D}$ and test point $\X_\text{test}$, data attribution for the $i^\text{th}$ training point $(\X_i, \Y_i)$ is a scalar estimate $\tau_i(\mathcal{A}, \mathcal{D}, \X_\text{test}) \in \R$ representing the influence of $(\X_i, \Y_i)$ on $\X_\text{test}$.
\end{defn}

To ground our discussion with a concrete example, we first introduce the conceptually most straightforward DA method, the Leave-One-Out (LOO) estimator. This computes the average prediction difference between a model trained on the original dataset vs one with a single training point excluded.

\begin{defn}
    (Leave-One-Out estimator) The LOO estimator of a learning algorithm $\mathcal{A}$, dataset $\mathcal{D}$ and test point $\X_\text{test}$, w.r.t. to training point $(\X_i, \Y_i)$ is given by
    $\tau_i(\mathcal{A}, \mathcal{D}, \X_\text{test}) = \mathbb{E}_{\theta \sim \mathcal{A}(\mathcal{D})} f(\X_\text{test}; \theta) - \mathbb{E}_{\theta_i \sim \mathcal{A}(\mathcal{D} \setminus \{(\X_i, \Y_i) \} )} f(\X_\text{test}; \theta_i)$
\end{defn}

The LOO estimator forms the conceptual basis for DA methods, but has several critical drawbacks.

% \textbf{Drawback: Attribution Computation Scales with Data Size.}
% % A critical challenge in data attribution is its substantial computational cost. From an abstract perspective, the definition of DA necessitates computing attributions for each training point individually, resulting in computational requirements that scale with the size of the training dataset $n$. This scaling becomes prohibitive in modern learning settings with large $n$. The computational burden can be even more severe in practice.
% Data attribution (DA) faces significant computational challenges due to its dependency on the size of the training dataset, $n$.
% For instance, the LOO estimator demands training at least $n+1$ models, with this number increasing significantly in non-convex settings due to Monte Carlo estimation for the expectation in Definition 2~\citep{jia2019towards}.
% Gradient-based methods, such as influence functions, aim to reduce attribution computation by avoiding retraining. However, these methods still require (1) computation of per-training-sample gradients w.r.t. parameters and (2) computation of the Hessian inverse of models parameters. Both these steps are computationally intensive, as (1) requires $n$ forward and backward passes, which is prohibitive when $n$ is in the billions, and (2) requires manipulating the Hessian matrix whose dimensions are $p \times p$ for a model $\theta \in \R^p$, which is again intractable when $p$ is in the billions.  

\textbf{Drawback: Computation Scales Intractably.}\hspace{5pt} Computationally, methods like the leave-one-out (LOO) estimator, which trains $n+1$ models, become impractical with large $n$. Additionally, gradient-based approaches like influence functions, still require (1) computation of per-training-sample gradients w.r.t. parameters ($n$ forward and backward passes) and (2) computation of the Hessian inverse of models parameters (dimensions of $p \times p$ for a model $\theta \in \R^p$).

\textbf{Drawback: Pointwise Attribution may be Ill-Defined.}\hspace{5pt} Recall that the LOO estimator involves repeatedly training models on \emph{nearly identical} training sets. However, as data scales, a single missing example is unlikely to lead to statistically significant change in model outputs, an intuition captured in literature via properties such as (1) stability of learning algorithms~\citep{elisseeff2005stability}, or (2) differential privacy~\citep{dwork2008differential}. %, which suggest that outputted models should not change when individual points are removed.%, owing to (1) model generalization and (2) privacy guarantees.
The conceptual basis for many methods, the LOO estimator, may be ill-defined under such conditions.

\textbf{Drawback: Focus on Individual Predictions Limits Scope.}\hspace{5pt}We may wish to identify training points that cause models to be inaccurate, non-robust, or unfair, all of which are ``bulk'' model properties. In these scenarios, DA has been adapted to analyze individually the test points that are inaccurate or non-robust, which is undesirable given (1) many model properties, such as fairness and f-measure, are non-decomposable \citep{narasimhan2015optimizing}, i.e., cannot be written in terms of contributions of individual test points, and (2) it is computationally wasteful to aggregate test point results over directly computing the metric. %We are thus interested in developing tools to directly analyze the impact of training data on bulk model behavior.

To resolve these, we propose two modifications to the DA framework, of (1) partitioning the training dataset into groups of training points and directly attributing model behaviour to these groups (similar data points may affect models in similar ways), and (2) expanding the scope of DA to focus beyond individual predictions to arbitrary ``property functions" of the model parameters, such as accuracy, robustness, and fairness. Collapsing groups to singletons or setting property functions to invididual loss subsumes standard DA. We now formally define these two new components:

\textbf{Group $\mathcal{Z}$}: Given a dataset $\mathcal{D}$, we define a partition of the dataset into $k$ groups such that $\mathcal{Z} = \{ \Z_0, \Z_1, ... \Z_k\}$, where each $\Z_j$ is a set of inputs $\X_i$ such that $\Z_j \cap \Z_i = \emptyset$ for $i \neq j$, and $\bigcup_i \Z_i = \mathcal{D}$. In general, the cardinality of each group $|\Z_i|$ may vary. A group size of 1 subsumes standard DA.

\textbf{Property function $g$}: Given a model with weights $\theta \in \R^p$, we define a property function $g(\cdot): \R^p \rightarrow \R$. Property functions generalize (1) pointwise functions like log probability of a given test point, (2) aggregate functions like accuracy on a test set. Given these, we are ready to define GGDA.

\begin{defn}
    (Generalized Group Data Attribution) Given a learning algorithm $\mathcal{A}$, dataset $\mathcal{D}$ with groups $\mathcal{Z}$ and property function $g$, GGDA wrt to the $j^\text{th}$ group $\Z_j$ estimates $\tau_j(\mathcal{A}, \mathcal{D}, \mathcal{Z}, g) \in \R$ representing the influence of group $\Z_j$ on model property $g$
\end{defn}

To ground this with a concrete example, we present the GGDA variant of the LOO estimator below. The idea is very similar to the usual LOO estimator, except here that we leave the $j^{th}$ group out, and measure the resulting change in the property function $g$.  

\begin{defn}
    The (GGDA LOO) estimator of a learning algorithm $\mathcal{A}$, dataset $\mathcal{D}$, groups $\mathcal{Z}$ and property function $g$, wrt to the $j^\text{th}$ group $\Z_j$ is given by
    $\tau_j(\mathcal{A}, \mathcal{D}, \mathcal{Z}, g) = \mathbb{E}_{\theta \sim \mathcal{A}(\mathcal{D})} g(\theta) - \mathbb{E}_{\theta_j \sim \mathcal{A}(\mathcal{D} \setminus Z_j )} g(\theta_j)$
\end{defn}

Comparing this to the usual LOO attributor, we observe that the GGDA variant requires training of $k+1$ models as opposed to $n+1$ models, which is advantageous when $k << n$. In summary, the main advantage of GGDA methods is that they \ul{scale as the number of groups $k$}, whereas DA methods \ul{scale with the number of data points $n$}. While extending LOO was fairly simple, it is, in general, non-trivial to extend arbitrary DA methods to GGDA methods, particularly in a way that makes the computation scale with the number of groups $k$, reflecting the advantage that group attribution offers. %For example, while \cite{koh2019accuracy} study group influence functions, they compute these group influences by summing the influences of individual training points, thus retaining the computational cost of standard DA.%In the next section, we present an example analysis with influence functions.% we shall propose GGDA variants of popular DA methods in a manner that exactly improves their computational efficiency.

==> neurips_format/related.tex <==
\textbf{Data Attribution} 
% Data attribution methods aim to quantify the influence of training samples on model predictions and can be broadly categorized into retraining-based and gradient-based approaches.
quantifies the influence of training samples on model predictions. 
One type is retraining-based, systematically retraining models with varying subsets of training data to measure sample influence. This includes Leave-One-Out (LOO) influence \cite{tukey1958bias}, and its extensions to subsets in Data Shapley \citep{ghorbani2019data,jia2019towards} and DataModels \citep{ilyas2022datamodels}, which can capture complex data interactions, but are computationally expensive due to reliance on retraining.
In contrast, gradient-based methods offer more scalable solutions, providing closed-form attribution scores.
Influence functions \citep{koh2017understanding} approximate the effect of upweighting a training sample on the loss function.
TracIn \citep{pruthi2020estimating} traces loss changes during the training process, and TRAK \citep{park2023trak} employs random projection to assess influence.
Gradient-based methods significantly reduce computation, but may suffer from performance degradation on non-convex neural networks due to reliance on convexity assumptions and Taylor approximations.

\textbf{Grouping in Data Attribution.}\hspace{5pt} Prior research has explored attributing effects to groups.
\cite{koh2019accuracy} analyzed influence functions for large groups, finding strong correlations between predicted and actual group effects on linear models (we focus on non-linear models).
\cite{basu2020second} developed a second-order influence function for better fidelity but at increased computational costs, whereas our focus is enhancing efficiency. \cite{ghorbani2019data} also touched on grouping data points as a strategy to handle large datasets, but our research systematically extends attribution methods to groups and experimentally validates that it is possible to generalize both re-training-based and gradient-based attribution methods.


%Their approach calculates Shapley values for predefined groups based on specific features, such as age or gender, in medical settings. This method provides a way to interpret the influence of subgroups with the same demographic features on model performance. In contrast, our GGDA framework does not rely on predefined groups or prior knowledge, offering more flexibility in group formation across various datasets and attribution tasks.

%Their method addresses the limitations of first-order approximations when removing larger groups of data points. Incorporating higher-order terms improved the correlation between computed influence values and ground truth, particularly for linear models. This approach emphasizes improving accuracy through increased computational complexity. In contrast, GGDA strikes a balance between attribution accuracy and computational efficiency, making it more practical for large-scale models and diverse attribution methods.


\textbf{Data Attribution Acceleration.}\hspace{5pt} Various approaches have been proposed to accelerate data attribution methods, including subsampling \citep{guo-etal-2021-fastif} and better gradient/Hessian approximations \citep{schioppa2022scaling}.
These techniques focus on optimizing existing attribution algorithms to improve computational efficiency.
While valuable, these methods are orthogonal to our GGDA framework, which fundamentally alters the attribution paradigm by considering groups of data points.
As such, GGDA can be combined with these techniques to achieve greater efficiency gains, highlighting its complementary nature.

==> sections/application.tex <==
Now that we have a setting in which data attribution is really accurate, we can start to think about the question: what applications can we now enable that weren't possible before because of shitty methods?

Some possibilities:

\begin{enumerate}
    \item Identifying corrupted training points, or points with corrupted labels, i.e., the points, which when removed, improved accuracy by the most amount
    \item Identifying the ``minimal training data" for achieving equivalent accuracy on the task
    \item Identify training examples that help OOD performance
    \item Identify the training examples that encode a particular concept for a model class
\end{enumerate}

For all these tasks, we only aim to compare within influence methods, and show that group methods outperform per-sample methods.

\pagebreak

==> sections/tables/noisy.tex <==
\begin{table}[h]
\caption{\small Mean noisy label detection AUC and runtimes for increasingly large Grad-K-Means groups, measured across all datasets and attribution methods. For HELOC, we display results from the ANN-S model.}
\label{tab:noisy}
\small
\begin{center}
\begin{tabular}{cccccccc}
\toprule
\multirow{2}*{Dataset} & \multirow{2}*{Attributor} & \multicolumn{5}{c}{Noisy Label Detection AUC / {\color{gray}Runtime (s)} per GGDA Group Size} \\
 &  & 1 (DA) & 4 & 16 & 64 & 256 \\
 
% \midrule  %%% LR
% \multirow{3}*{HELOC} & TracIn & 0.555 / {\color{gray}7.44} & 0.545 / {\color{gray}1.96} & 0.539 / {\color{gray}0.54} & 0.541 / {\color{gray}0.18} & 0.539 / {\color{gray}0.08} \\
% & Influence (Fisher) & 0.614 / {\color{gray}7.43} & 0.581 / {\color{gray}1.95} & 0.558 / {\color{gray}0.52} & 0.520 / {\color{gray}0.17} & 0.512 / {\color{gray}0.08} \\
% & Influence (LiSSA) & 0.575 / {\color{gray}13.54} & 0.572 / {\color{gray}7.38} & 0.571 / {\color{gray}5.78} & 0.572 / {\color{gray}5.39} & 0.573 / {\color{gray}5.30} \\

% \midrule  %%% ANN_S
% \multirow{3}*{HELOC} & TracIn & 0.580 / {\color{gray}10.6} & 0.572 / {\color{gray}2.95} & 0.568 / {\color{gray}0.90} & 0.566 / {\color{gray}0.40} & 0.566 / {\color{gray}0.28} \\
% & Inf. (Fisher) & 0.604 / {\color{gray}9.25} & 0.582 / {\color{gray}2.51} & 0.552 / {\color{gray}0.76} & 0.495 / {\color{gray}0.34} & 0.510 / {\color{gray}0.23} \\
% & Inf. (LiSSA) & 0.650 / {\color{gray}18.5} & 0.631 / {\color{gray}11.9} & 0.627 / {\color{gray}10.2} & 0.621 / {\color{gray}9.77} & 0.620 / {\color{gray}9.65} \\
% & TRAK & 0.504 / {\color{gray}46.4} & 0.549 / {\color{gray}12.0} & 0.528 / {\color{gray}3.92} & 0.512 / {\color{gray}1.22} & 0.503 / {\color{gray}0.77} \\

% \midrule  %%% ANN_M
% \multirow{3}*{HELOC} & TracIn & 0.597 / {\color{gray}11.44} & 0.560 / {\color{gray}3.44} & 0.553 / {\color{gray}1.29} & 0.549 / {\color{gray}0.75} & 0.550 / {\color{gray}0.60} \\
% & Inf. (Fisher) & 0.597 / {\color{gray}13.39} & 0.571 / {\color{gray}4.05} & 0.563 / {\color{gray}1.47} & 0.536 / {\color{gray}0.81} & 0.533 / {\color{gray}0.63} \\
% & Inf. (LiSSA) & 0.636 / {\color{gray}24.10} & 0.601 / {\color{gray}16.70} & 0.595 / {\color{gray}14.43} & 0.592 / {\color{gray}13.75} & 0.592 / {\color{gray}13.70} \\
% \midrule

\midrule
\multirow{3}*{MNIST} & TracIn & 0.637 / {\color{gray}208} & 0.646 / {\color{gray}55.9} & 0.650 / {\color{gray}18.1} & 0.642 / {\color{gray}8.18} & 0.529 / {\color{gray}5.69} \\
& Inf. (Fisher) & 0.509 / {\color{gray}287} & 0.551 / {\color{gray}90.7} & 0.586 / {\color{gray}27.8} & 0.554 / {\color{gray}9.49} & 0.502 / {\color{gray}4.58} \\
& Inf. (LiSSA) & 0.640 / {\color{gray}220} & 0.647 / {\color{gray}71.7} & 0.647 / {\color{gray}35.2} & 0.639 / {\color{gray}25.5} & 0.534 / {\color{gray}23.2} \\
& TRAK & 0.495 / {\color{gray}868} & 0.501 / {\color{gray}240} & 0.502 / {\color{gray}87.7} & 0.504 / {\color{gray}23.9} & 0.501 / {\color{gray}33.0} \\

\midrule
\multirow{3}*{CIFAR-10} & TracIn & 0.700 / {\color{gray}558} & 0.702 / {\color{gray}172} & 0.704 / {\color{gray}59.0} & 0.705 / {\color{gray}31.6} & 0.707 / {\color{gray}24.1} \\
& Inf. (Fisher) & 0.630 / {\color{gray}497} & 0.614 / {\color{gray}172} & 0.602 / {\color{gray}69.8} & 0.573 / {\color{gray}40.5} & 0.569 / {\color{gray}35.0} \\
& Inf. (LiSSA) & 0.656 / {\color{gray}835} & 0.657 / {\color{gray}544} & 0.661 / {\color{gray}468} & 0.678 / {\color{gray}452} & 0.685 / {\color{gray}447} \\
& TRAK & 0.501 / {\color{gray}1814} & 0.490 / {\color{gray}674} & 0.486 / {\color{gray}319} & 0.482 / {\color{gray}210} & 0.497 / {\color{gray}188} \\

% \midrule
% \multirow{2}*{QNLI} & TracIn & 0.543 / {\color{gray}1743} & 0.539 / {\color{gray}427} & 0.537 / {\color{gray}172} & 0.536 / {\color{gray}136} & 0.536 / {\color{gray}119} \\
% & Inf. (Fisher) & 0.667 / {\color{gray}2207} & 0.695 / {\color{gray}493} & 0.684 / {\color{gray}187} & 0.605 / {\color{gray}145} & 0.508 / {\color{gray}135} \\
% & Inf. (LiSSA) & 0.501 / {\color{gray}2043} & 0.504 / {\color{gray}686} & 0.489 / {\color{gray}395} & 0.490 / {\color{gray}403} & 0.512 / {\color{gray}392} \\
% & TRAK & 0.500 / {\color{gray}4947} & 0.498 / {\color{gray}1698} & 0.497 / {\color{gray}841} & 0.507 / {\color{gray}739} & 0.502 / {\color{gray}788} \\

\midrule
\end{tabular}
\end{center}
\end{table}
